Variational Bayesian Inference for Time-Varying Massive MIMO Channels: Estimation and Detection

Massive multiple-input multiple-output (MIMO) stands as a key technology for advancing performance metrics such as data rate, reliability, and spectrum efficiency in the fifth generation (5G) and beyond of wireless networks. However, its efficiency depends greatly on obtaining accurate channel state information. This task becomes particularly challenging with increasing user mobility. In this paper, we focus on an uplink scenario in which a massive MIMO base station serves multiple high-mobility users. We leverage variational Bayesian(VB) inference for joint channel estimation and data detection(JED), tailored for time-varying channels. In particular, we use the VB framework to provide approximations of the true posterior distributions. To cover more real-world scenarios, we assume the time correlation coefficients associated with the channels are unknown. Our simulations demonstrate the efficacy of our proposed VB-based approach in tracking these unknown time correlation coefficients. We present two processing strategies within the VB framework: online and block processing strategies. The online strategy offers a low-complexity solution for a given time slot, requiring only the knowledge of the parameters/statistics within that time slot. In contrast, the block processing strategy focuses on the entire communication block and processes all received signals together to reduce channel estimation errors. Additionally, we introduce an interleaved structure for the online processing strategy to further enhance its performance. Finally, we conduct a comparative analysis of our VB approach against the linear minimum mean squared error(LMMSE), the Kalman Filter(KF), and the expectation propagation(EP) methods in terms of symbol error rate(SER) and channel normalized mean squared error(NMSE). Our findings reveal that our VB framework surpasses these benchmarks across the performance metrics.

==> Sections/Acknowledgment.tex <==
{This work was supported by the U.S. Department of Defense (DoD) under Grant W911NF-23-1-0226 and by the National Science Foundation (NSF) under Grant CCF-2225576.}

==> Sections/Background.tex <==
%\subsection{Variational Bayes for Approximate Inference}

%\sncomment{As you mentioned, VB is a known approach. So, I was wondering if we would summarize this background section by citing the reference of ELBO and pointing out $q_i^{\star}(x_i)$ as \eqref{eq:q_start_prop}?} \textcolor{blue}{You can help to shorten this part from your perspective. That'd be better than I rewrite the part on my own.}
 
	This section provides a summary of the variational Bayes (VB) method for approximate inference. Denote the set of all observed variables by $\mb{y}$ and set of $L$ latent variables and parameters by $\mb{x}$. For detection purposes, it is essential to find the posterior $p(\mb{x}|\mb{y})$, which is computationally intractable. To tackle this issue, the VB method was introduced to obtain a distribution $q(\mb{x})$ with its own setting of variational parameters within a family $\mc{Q}$ of densities such that $q(\mb{x})$ approximates $p(\mb{x}|\mb{y})$. To do so, the VB method defines the following optimization problem using the Kullback-Leibler (KL) divergence
from $q(\mb{x})$ to $p(\mb{x}|\mb{y})$.
	\begin{eqnarray}
 \label{eq:opt_KL}
		q^{\star}(\mb{x}) = \argmin_{q(\mb{x}) \in \mc{Q}}\; \mr{KL}\big(q(\mb{x}) \|p(\mb{x}|\mb{y}) \big),
	\end{eqnarray}
	where $q^{\star}(\mb{x})$ is the optimal variational distribution and
	\begin{eqnarray}
\mr{KL}\big(q(\mb{x}) \|p(\mb{x}|\mb{y}) \big) = \E_{q(\mb{x})} \big[\ln q(\mb{x}) \big] - \E_{q(\mb{x})} \big[\ln p(\mb{x}|\mb{y})\big]. 
	\end{eqnarray}
 
	In~\cite{Bishop-2006}, the authors showed that the optimization problem in~\eqref{eq:opt_KL} is equivalent to the following maximization problem.
 \begin{eqnarray}
 \label{eq:opt_ELBO}
		q^{\star}(\mb{x}) = \argmax_{q(\mb{x}) \in \mc{Q}}\; \big\{\E_{q(\mb{x})} \left[\ln p(\mb{x},\mb{y})\right] - \E_{q(\mb{x})} \left[\ln q(\mb{x}) \right]\big\},
	\end{eqnarray}
where the objective function is referred to as the evidence lower bound ($\mr{ELBO}$). Here,~\eqref{eq:opt_ELBO} is maximized when $q(\mb{x}) = p(\mb{x}|\mb{y})$. Due to the fact that obtaining the true posterior distribution is intractable, it is more practical to consider a restricted family of distribution $q(\mb{x})$. Hence, this work focuses on the \emph{mean-field variational family}, which is defined as follows:	\begin{eqnarray}\label{mean-field}
		q(\mb{x}) = \prod_{i=1}^Lq_i(x_i),
	\end{eqnarray}
	where the latent variables are mutually independent and each governed by a distinct factor in the variational density. %Among all distribution $q(\mb{x})$ having the form \eqref{mean-field}, we seek the distribution for which  $\mr{ELBO}(q)$ is maximized. %Substituting \eqref{mean-field} into $\mr{ELBO}(q)$, and considering one of the factor $x_i$, one has
	%	\begin{eqnarray}
		%		\mr{ELBO}(q) = -\mr{KL}\big(q_i(x_i) \|\tilde{p}(x_i,\mb{y}) \big) +\mr{const},
		%	\end{eqnarray}
	%	where the $\mr{const}$ term does not depend on $x_i$ and a new distribution 
	%	$\tilde{p}(x_i,\mb{y})$ is defined as
	%	\begin{eqnarray}
		%		\ln\tilde{p}(x_i,\mb{y}) &=& \E_{q_{-i}(\mb{x}_{-i})}\big[\ln p (\mb{x},\mb{y})\big] + \mr{const}. \nonumber \\
		%		&=&  \big\langle{\ln p (\mb{y}|\mb{x}) + \ln p(\mb{x})\big\rangle} + \mr{const}.
		%	\end{eqnarray}
	%	Here $\E_{q_{-i}(\mb{x}_{-i})}[\cdot]$ and $\lr{\cdot}$ denote the expectation with respect to all latent variables except $x_i$ using the currently fixed variational density $q_{-i}(\mb{x}_{-i}) = \prod_{j\neq i} q_{j}(x_{j})$. 
	%	Thus, maximizing $\mr{ELBO}(q)$ with respect to $x_i$ is equivalent to minimizing the KL divergence between $q_i(x_i)$ and $\tilde{p}(x_i,\mb{y})$, and the minimum occurs when $q_i(x_i) = \tilde{p}(x_i,\mb{y})$. Thus, we obtain a general expression for the optimal solution of the variational density $q_i(x_i)$ as
	%	\begin{eqnarray}
		%		q_i^{\star}(x_i) \propto \mr{exp}\left\{\big\langle{\ln p (\mb{y}|\mb{x}) + \ln p(\mb{x})\big\rangle}\right\}.
		%	\end{eqnarray}
	The general expression for the optimal solution of the variational density $q_i(x_i)$ can be obtained as \cite{Bishop-2006}:
	\begin{align}
 \label{eq:q_start_prop}
		q_i^{\star}(x_i) &\propto \mr{exp}\left\{\big\langle{\ln p (\mb{y},\mb{x})\big\rangle}\right\} \\ \nonumber
  &\propto \mr{exp}\left\{\big\langle{\ln p (\mb{y}|\mb{x}) + \ln p(\mb{x})\big\rangle}\right\},
	\end{align}
	where $\lr{\cdot}$ represents the expectation with respect to all latent variables except $x_i$ using the currently fixed variational density $q_{-i}(\mb{x}_{-i}) = \prod_{j=1, j\neq i}^{L} q_{j}(x_{j})$. By sequentially updating $q_i^{\star}(x_i)$ in an iterative manner for all $j$, the objective function of~\eqref{eq:opt_ELBO} is monotonically enhanced. This forms the fundamental principle of the \emph{Coordinate Ascent Variational Inference (CAVI)} algorithm, which ensures convergence to at least a local optimum solution for the optimization problem in~\eqref{eq:opt_ELBO} \cite{Wainwright-2008}.


	% \subsection{Data Detection with Perfect CSIR}
	% Genie-aided CSI is available at the BS. 
	
	% \subsubsection{Linear Detectors} \textcolor{blue}{We can move this to the simulation, that we use LMMSE for the channel estimation and LMMSE detection.}
	% \sncomment{Can we remove this subsection for LMMSE since it is a well-known approach, and instead, mention its pros and cons in words in the Introduction and then use it as a benchmark in simulations?} A linear MMSE estimate of the data symbol vector $\mb{x}$ can be obtained as
	% \begin{eqnarray}
	% 	\hat{\mb{x}}_t = \mb{H}_t^H\big({\mb{H}}_t{\mb{H}}_t^H + N_0\mb{I}_M\big)^{-1}\mb{y}_t.
	% \end{eqnarray}
	% The linear MMSE estimate $\hat{\mb{x}}$ is then projected onto the constellation $\mc{S}$ on a per-user basis to obtain the final estimate of the data symbol vector $\mb{x}$. 
	
	% \subsubsection{Nonlinear Detectors}
	% We consider a VB detector

